Depth from Coupled Optical Differentiation

We propose depth from coupled optical differentiation, a low-computation passive-lighting 3D sensing mechanism. It is based on our discovery that per-pixel object distance can be rigorously determined by a coupled pair of optical derivatives of a defocused image using a simple, closed-form relationship. Unlike previous depth-from-defocus (DfD) methods that leverage spatial derivatives of the image to estimate scene depths, the proposed mechanism's use of only optical derivatives makes it significantly more robust to noise. Furthermore, unlike many previous DfD algorithms with requirements on aperture code, this relationship is proved to be universal to a broad range of aperture codes. We build the first 3D sensor based on depth from coupled optical differentiation. Its optical assembly includes a deformable lens and a motorized iris, which enables dynamic adjustments to the optical power and aperture radius. The sensor captures two pairs of images: one pair with a differential change of optical power and the other with a differential change of aperture scale. From the four images, a depth and confidence map can be generated with only 36 floating point operations per output pixel (FLOPOP), more than ten times lower than the previous lowest passive-lighting depth sensing solution to our knowledge. Additionally, the depth map generated by the proposed sensor demonstrates more than twice the working range of previous DfD methods while using significantly lower computation.

==> theory-deprecated.tex <==
\section{Theory}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6\textwidth]{figs/1cod.pdf}
    \caption{(a) Principle of coupled optical differentiation. Consider a thin lens camera with adjustable optical power $\rho$, aperture scale $\mathnormal{A}$, and sensor distance $Z_s$. The image it captures is a function of these optical parameters, denoted as $I(\rho, \mathnormal{A}, Z_s)$. In this work, we show that the ratio of the intensity derivative w.r.t. two optical parameters, e.g. $I_\mathnormal{A} / I_\rho$, reveals the object depth $Z$ at each pixel through closed-form solutions.
    % The optics transform each uniform-irradiance point light source to a defocused pattern on the photosensor called the point spread function (PSF), denoted as $k(x,y)$. The width of the PSF depends on the optical parameters $\rho, \mathnormal{A}, Z_s$ and the depth of the point $Z$. 
    (b) Images of the same object captured with different optical parameters. By adjusting the optical parameters $\rho, \mathnormal{A}, Z_s$, the camera can capture images $I$ of the object with different defocus levels. (c) Pixel intensity vs. optical power  $\rho$. The colored markers indicate the intensities of corresponding image pixels in (b). The intensity varies in textured regions,  e.g., pixel $\bullet$, when the object is out of the depth-of-field (DoF). Meanwhile, the intensity is close to constant in textureless regions, such as at pixel $\blacklozenge$. (d) Pixel intensity vs. aperture scale $\mathnormal{A}$. The plot visualizes the intensity of pixel $\bullet$ as a function of aperture scale $\mathnormal{A}$ under three different optical powers, $\rho-\Delta\rho, \rho$,  and $\rho+\Delta\rho$. The image $I(\rho+\Delta\rho, \mathnormal{A}, Z_s)$ is in focus (see b). Thus, the pixel intensity of $I(\rho+\Delta\rho, \mathnormal{A}, Z_s)$ stays approximately constant w.r.t. the aperture scale $\mathnormal{A}$. Similar to (c), there is little intensity variation in textureless regions, e.g., the red curve. }
    % At a fixed pixel varies w.r.t. the optical power $\rho$ (c) and aperture scale $\mathnormal{A}$ (d).  
    % The intensity variation is the most significant in textured regions, such as at pixels indicated by $\bullet$. At textureless regions, e.g., $\blacklozenge$, the intensity remains constant w.r.t. the optical parameters. Also, when the image is in focus, such as $I(\rho+\Delta \rho)$, the image intensity varies slowly w.r.t. the aperture scale $\mathnormal{A}$. 
    % In this work, we show that the ratio of the intensity derivative w.r.t. two optical parameters reveals the object depth $Z$ at the pixel. Thus, the magnitude of the image derivative determines the signal-to-noise ratio of the depth estimation. }
    \label{fig:principle}
\end{figure}

\subsection{Image Formation Model}
As shown in Fig.~\ref{fig:principle}, we consider a thin-lens camera imaging a front-parallel object with spatially-varying intensity $T(x,y)$ located a constant depth $Z$ from the camera. The captured image can be modeled with a pinhole projection followed by defocus blur as:
\begin{align}
    I(x,y) = k(x,y;Z) * T\left(-\frac{Z}{Z_s}x,-\frac{Z}{Z_s}y\right),
\label{eq:ifm}
\end{align}
where $k(x,y;Z)$ is the camera's point spread function (PSF) corresponding to object distance $Z$. The PSF is a scaled version of the aperture transmittance profile $\kappa(x,y)$, with the scale $\mathnormal{A}$ determined by the optical parameters of the camera: the optical power $\rho$, the aperture diameter $\mathnormal{A}$, and the distance $Z_s$ between the aperture and the sensor, as
\begin{align}
     k(x,y;Z) = \frac{1}{A^2\sigma^2(Z, \rho, Z_s)}\cdot \kappa\left(\frac{x}{\mathnormal{A} \cdot \sigma(Z, \rho, Z_s)},\frac{y}{\mathnormal{A} \cdot \sigma(Z, \rho, Z_s)}\right).
     \label{eq:k}
\end{align}
Specifically, $\sigma$ indicates the defocus level of the PSF:
\begin{align}
    \sigma(Z, \rho, Z_s) = Z_s\left(\rho - \frac{1}{Z}\right) + 1.\label{eq:sig}
\end{align}
For objects with slowly varying depth, Eq.~\ref{eq:ifm} can still be used by approximating the object as patch-wise fronto-parallel~\cite{guo2019compact, guo2017focal, alexander2018focal}. 

% Therefore, by estimating the defocus level 
% The objective of the proposed algorithm is to predict the object distance $Z$ by estimating the defocus level $\sigma$ from the measured images $I(x,y)$. 

% For simplicity, we skip the pixel-notation $(x,y)$, as most calculations in this manuscript are per pixel unless noted. 

% For objects that are not fronto-parallel, we assume 
% Eq.~\ref{eq:ifm} can still be used when the distance map of the object varies slowly. 

% can be approximately generalized to model the image formation process when the PSF of an object varies slowly, which 

% the image of a point source with distance $Z$, or the point spread function (PSF), is $k(x,y;Z, \rho, \kappa, Z_s)$:
% \begin{align}
%     k(x,y;Z, \rho,\kappa,Z_s) = \kappa\left(\frac{x}{\sigma(Z, \rho, Z_s)},\frac{y}{\sigma(Z, \rho, Z_s)}\right),
% \end{align}
% where the term $\sigma$ indicates the magnification of the pupil function and can be thought of as the defocus level. According to Thin-lens' Law, the term $\sigma$ can be calculated as:
% \begin{align}
%     \sigma(Z, \rho, Z_s) = Z_s\left(\rho - \frac{1}{Z}\right) + 1.
% \end{align}
% The image of a fronto-parallel texture target at a distance $Z$ is the spatial convolution of the PSF with the pinhole image $P(x,y)$:
% \begin{align}
%     I(x,y;Z, \rho,\kappa,Z_s) = k(x,y;Z, \rho,\kappa,Z_s) * P(x,y).
%     \label{eq:img_formation}
% \end{align}
% Compared to Focal Track / Focal Flow, the derivation does not specifically assume the shape of the pupil function. 

\subsection{Depth Estimation}
\label{secsec:depth}

Our objective is to estimate object depth $Z$ from changes in image brightness $I(x,y)$ caused by changes in defocus level $\sigma$. From Eq.~\ref{eq:ifm} we observe that the partial derivatives, denoted by subscripts, of the image with respect to each optical parameter, $\rho, Z_s, \mathnormal{A}$, are all proportional:
\begin{align}
   \mathnormal{A} \cdot I_{\mathnormal{A}} = \frac{\sigma}{\sigma_{Z_s}} \cdot I_{Z_s} = \frac{\sigma}{\sigma_{\rho}} \cdot I_{\rho}  = -(xk_x +yk_y) * T.\label{eq:ratio}
\end{align}
Prior work has established that the final expression, interpreted as a defocus residual on brightness constancy, can only be observed from spatial derivatives of defocused images if the blur is Gaussian~\cite{alexander2018focal}. However, we observe below that by comparing the image changes across a coupled pair of optical changes, the depth is revealed for any $k$. Further,  we no longer require spatial neighborhoods of pixels for depth estimation, shrinking both computational cost and sensitivity to local depth variations. Dropping the notation $(x,y)$ for simplicity, Eqs.~\ref{eq:sig} \& \ref{eq:ratio} give
three per-pixel equations to estimate the object depth $Z$ from
any two of the image derivatives $I_{\mathnormal{A}}, I_{Z_s}, I_{\rho}$:
\begin{align}
    Z &= \frac{\frac{I_{Z_s}}{I_\mathnormal{A}} - \mathnormal{A}}{(Z_s\rho + 1)\cdot \frac{I_{Z_s}}{I_\mathnormal{A}} - \mathnormal{A}\rho}, \label{eq:ZsSigma}\\
    Z &= \frac{Z_s}{(Z_s\rho - 1) - \mathnormal{A} Z_s \cdot \frac{I_\mathnormal{A}}{I_\rho}}, \label{eq:rhoSigma} \\
    Z &= \frac{1}{\rho - Z_s \frac{I_{Z_s}}{I_\rho}}
    \label{eq:Zsrho}.
\end{align}
Applying any one of these equations at each pixel in parallel will generate a depth map of the scene, with only two divides and a few adds and multiplies per pixel.


Each of Eq.~\ref{eq:ZsSigma}-\ref{eq:Zsrho} requires a pair of image derivatives that can be measured by computing the finite difference of the images captured under different defocus conditions, e.g.,
\begin{align}
    I_{\rho} &= \frac{I(\rho+\Delta \rho) - I(\rho - \Delta \rho)}{2\Delta \rho},
    \label{eq:fin}
\end{align}
with a coupled incremental change of optical parameters $(\Delta\mathnormal{A}, \Delta Z_s)$, $(\Delta\mathnormal{A}, \Delta \rho)$, or $(\Delta\rho, \Delta Z_s)$. Therefore, we name this family of depth estimation techniques \textit{depth from coupled optical differentiation}. Throughout the paper, we denote the image derivatives estimated from the finite difference as $I_\rho, I_\mathnormal{A}, $ and $I_{Z_s}$, and use $I^*_\rho, I^*_\mathnormal{A}, $ and $I^*_{Z_s}$ to represent true, noiseless image derivatives.
%\begin{align}
    %I_{Z_s} &= \lim_{\Delta Z_s\rightarrow 0} \frac{I(Z_s+\Delta Z_s) - I(Z_s - \Delta Z_s)}{2\Delta Z_s}, \\
    %I_{\rho} &= \lim_{\Delta \rho\rightarrow 0} \frac{I(\rho+\Delta \rho) - I(\rho - \Delta \rho)}{2\Delta \rho}, \\
    %I_{\mathnormal{A}} &= \lim_{\Delta \mathnormal{A}\rightarrow 0} \frac{I(\mathnormal{A}+\Delta \mathnormal{A}) - I(\mathnormal{A} - \Delta \mathnormal{A})}{2\Delta \mathnormal{A}}.
%\end{align}
The measurements needed by finite differences require physical adjustments to the camera. As shown in Fig.~\ref{fig:principle}a, the differentiation of the optical power $\Delta \rho$ or the sensor distance $\Delta Z_s$ can be achieved using a focus-tunable lens or a focus motor, respectively. The differentiation of the aperture scale $\Delta A$ is less straightforward to be realized. If the imaging system uses a circular aperture, i.e., the aperture transmittance profile $\kappa(x,y)$ is a 2D pillbox function with radius $\frac{1}{\pi}$:
\begin{align}
    \kappa(x,y) = \frac{1}{\pi}\left(\sqrt{x^2 + y^2} < 1\right),
    \label{eq:pillbox}
\end{align}
we can use a motorized iris to `equivalently' change the aperture scale $A$ by normalizing the brightness of the captured image:
\begin{align}
    I(\mathnormal{A} + \Delta \mathnormal{A}) = \left(\frac{\mathnormal{A}}{\mathnormal{A} + \Delta \mathnormal{A}}\right)^2 \Tilde{I}(\mathnormal{A}+\Delta \mathnormal{A}),
    \label{eq:bright_adjust}
\end{align}
where $\Tilde{I}(\mathnormal{A}+\Delta \mathnormal{A})$ the raw captured image with aperture scale $\mathnormal{A}+\Delta \mathnormal{A}$. In Sec.~\ref{}, we demonstrate a sensor prototype that can perform coupled optical differentiation $(\Delta\mathnormal{A}, \Delta \rho)$ using a custom optical assembly with an off-the-shelf motorized iris and deformable lens.  

% as with a motorized iris, a focus motor, or a focus-tunable lens. Therefore, we name this family of depth estimation techniques \textit{depth from coupled optical differentiation}. 

\subsection{Failure Cases and Mitigation}
\label{secsec:fail}

There are two failure cases for depth sensing equations (Eq.~\ref{eq:ZsSigma}-\ref{eq:Zsrho}.) First, the proposed method fails in image regions that lack spatial variation in intensity, as any triangulation-based method does. This is illustrated in Fig.~\ref{fig:principle}c-d, where the image intensity stays constant with respect to the change of optical parameters $\rho$ and $\mathnormal{A}$ at a pixel in the textureless region. Thus, both image derivatives $I_\rho$ and $I_\mathnormal{A}$ in Eq.~\ref{eq:rhoSigma} becomes zero. The situation is similar for Eq.~\ref{eq:ZsSigma} and \ref{eq:Zsrho}. Fortunately, this situation can be detected directly from the values of image derivatives $I_\rho, I_\mathnormal{A}, I_{Z_s}$, which can inform confidence of the depth estimation to filter out bad pixels. We seek a per-pixel, computationally inexpensive confidence metric high in regions of strong image derivative signals $I_\rho, I_\mathnormal{A}, I_{Z_s}$ and vice versa.
% To this end, we require that optical changes lead to image changes, with a saturation in confidence once sufficient image derivative signal has been observed.

Second, 
% The second case is practically related to the implementation. In practice, 
the finite difference estimation of image derivatives $I_\rho, I_{Z_s},$ and $I_{\mathnormal{A}}$ becomes inaccurate when the captured images are close to focus. There are several reasons that cause this phenomenon. This can also be witnessed in Fig.~\ref{fig:principle}c-d. When changing the optical power $\rho$, the pixel intensity $I$ is constant when the object is in the depth-of-field (Fig.~\ref{fig:principle}c.) Besides, the pixel intensity $I$ also remains constant w.r.t. the aperture scale $\mathnormal{A}$ if the object is in focus (Fig.~\ref{fig:principle}c.) This indicates that both image derivatives $I_\rho$ and $I_\mathnormal{A}$ go to zero when the object is in focus, and Eq.~\ref{eq:rhoSigma} degenerates. Thankfully, once again, these scenarios can be identified from the values of image derivatives $I_\rho, I_{Z_s}$, as they are close to zero when the image is close to focus. 

% First, the image intensity $I$ becomes a nonlinear function of the optical parameters when the image is close to focus. This can be seen in Fig.~\ref{fig:principle}c; the intensity of the blue curve becomes less linear when the targe enters the depth of field. \qg{More clarification.}
% the finite difference estimation of the image derivatives $I_\rho$ and $I_{\mathnormal{A}}$ could deviate from the true value $I_\rho^*$ and $I_{\mathnormal{A}}^*$ due to the nonlinearity. 
% % This problem is less severe to the estimation of $I_\mathnormal{A}$, as the image intensity $I$ is typically a linear function with respect to the aperture dimension $\mathnormal{A}$ (Fig.~\ref{}.) 
% Second, all image derivatives with respect to optical parameters degrade to zero as the images become in focus, as shown in Fig.~\ref{fig:principle}c. Thus, Eq.~\ref{eq:ZsSigma}-\ref{eq:Zsrho} degenerates when the object is at the focal plane. Thankfully, once again, these scenarios can be identified from the values of image derivatives $I_\rho, I_{Z_s}$, as they are close to zero when the image is close to focus. 

% can also be identified from the values of the image derivatives, as image derivatives $I_\rho, I_\mathnormal{A}, I_{Z_s}$ are small when the image is close to focus. 

% shape of $I_\rho, I_\mathnormal{A}$ 

% The second case is unique to Eq.~\ref{eq:rhoSigma}. As visualized in Fig.~\ref{}b, the image derivatives with respect to optical power and aperture dimension $I_\rho$ and $I_\mathnormal{A}$ both go to zero when the object is in focus. 

% Fortunately, these situations can be detected directly from the image derivative measurements, which can inform confidence estimates to filter out bad pixels. We seek a per-pixel, computationally inexpensive confidence metric high in regions of strong defocus signal. To this end, we require that optical changes lead to image changes, with a saturation in confidence once sufficient signal has been observed. Thus, we define the confidence value $C$ at each pixel $(x,y)$ from the image derivatives used in the depth estimation in Eq.~\ref{eq:ZsSigma}-\ref{eq:Zsrho}. In practice, we calculate the confidence for each depth equation

Combining both situations, we can identify and filter out pixels with failed depth estimation using a simple, per-pixel confidence metric based on the image derivatives. For each of the depth estimation equations in Eq.~\ref{eq:ZsSigma}-\ref{eq:Zsrho}, we calculate the confidence as:
\begin{align}
    C_{(\text{Eq.}~\ref{eq:ZsSigma})} &= I_{Z_s}^2, \label{eq:ZsSigma_C}\\
    C_{(\text{Eq.}~\ref{eq:rhoSigma})} &= C_{(\text{Eq.}~\ref{eq:Zsrho})} = I_{\rho}^2. \label{eq:rhoSigma_C} 
\end{align}
We filter out bad depth estimations using a pre-determined, fixed confidence threshold $C_{\text{thre}}$: 
% Thus, in practice, the confidence can be calculated with a multiply operation, and we can inverse the sigmoid function to the confidence threshold and filter pixels based on:
\begin{align}
    Z = \begin{cases}
        Z, \quad C > C_{\text{thre}} \\
        \text{unconfident}, \quad \text{otherwise}.
    \end{cases}
\end{align}
% For example, we can calculate the confidence for each depth equation:
% \begin{align}
%     C = \text{sigmoid}\left(I_{\rho}^2\right).
% \end{align}
We show in Sec.~\ref{secsec:sim-conf} and Sec. XX the effectiveness of this simple confidence metric to filter out erroneous depth estimations in simulation and real experiments.

Additionally, the term $xk_x + yk_y$ in equation \ref{eq:ratio} can generate difficulties for blur kernels $k$ with sharp edges, which produce ill-defined spatial derivatives. The multiplication with the variables of convolution (i.e. that the terms are of the form $xk_x$ instead of simply $k_x$) complicates the process of moving the differentiation onto the texture through the associativity of convolution. In reality, blur kernels are never perfectly sharp due to effects such as diffraction that we do not explicitly model here. We perform a simulation study to determine the optimal shape of blur kernels $k$ in Sec.~\ref{secsec:psf}. 

% In practice, smoother blur kernels such as Gaussians outperform pillbox kernels because [explanation once I've seen some examples]. Figure XX shows [examples using Gaussian and pillbox results, with and without diffraction - can use confidence because we've already defined this]. [Comment]

%\subsection{Failure Cases}

% \qg{Emma, can you discuss when Eq. 7-9 does not hold? Such as when $\kappa$ is not differentiable or if there is a problem at edge?}
% \ea{I restructured things a little and suggest an analysis, let's discuss :)}
% \qg{I love how you reorg everything! Yes, let's talk more about analysis. I personally want to make it a separate section and want to prove something like the optimal aperture code with the highest SNR. Not sure if it is possible.}

% \subsection{Coupled Optical Differentiation}




% \qg{Add a figure here to show the three different optical differentiations}

% Depending on the allowance of the maximum number of images that can be captured per every depth estimation, the image derivatives can be estimated more accurately with more than two captured images via higher-order finite differences. 

%\qg{Summarize the significance of this method. The method is aperture-code invariant and texture invariant. Draw a comparison with DfDD here, which only works for Gaussian aperture code.}

% \subsection{Confidence}


